The hyperboloidal foliation method

The Hyperboloidal Foliation Method presented in this monograph is based on a (3+1)-foliation of Minkowski spacetime by hyperboloidal hypersurfaces. It allows us to establish global-in-time existence results for systems of nonlinear wave equations posed on a curved spacetime and to derive uniform energy bounds and optimal rates of decay in time. We are also able to encompass the wave equation and the Klein-Gordon equation in a unified framework and to establish a well-posedness theory for nonlinear wave-Klein-Gordon systems and a large class of nonlinear interactions. The hyperboloidal foliation of Minkowski spacetime we rely upon in this book has the advantage of being geometric in nature and, especially, invariant under Lorentz transformations. As stated, our theory applies to many systems arising in mathematical physics and involving a massive scalar field, such as the Dirac-Klein-Gordon system. As it provides uniform energy bounds and optimal rates of decay in time, our method appears to be very robust and should extend to even more general systems.

==> check.tex <==
%% Usage: Latex check.tex
%%
%% Utility to test if all the files required for WSPC book 9x6 project
%% are available in your present LaTeX path.
%%
%% - ws-book9x6.cls
%% - ws-crop9x6.sty
%% - ws-book-har.sty
%% - ws-book-var.sty
%% - ws-book-har.bst
%% - ws-book-van.bst
%% - ws-multind.sty
%% - ws-book-thm.sty
%% - rotating.sty
%% - crop.sty
%% - hyperref.sty
%% - boxedminipage.sty
%% - makeidx.sty

\newif\onerror
\typeout{*}
\typeout{1. Searching for LaTeX2e ... }
\ifx\documentclass\undefined
 \typeout{*}
 \typeout{* Fatal error occurred:}
 \typeout{*}
 \typeout{* The WS Book class can only be used with LaTeX2e}
 \typeout{*}
 \typeout{* Stopping...}
 \expandafter\stop
\else
 \typeout{   ... ok}
\fi

\def\next#1/#2/#3\next{#1#2}
\typeout{ }
\typeout{2.  Searching for LaTeX2e version ... }
\ifnum\expandafter\next\fmtversion\next<199612 \relax
 \typeout{*}
 \typeout{* Fatal error occurred:}
 \typeout{*}
 \typeout{* Your LaTeX version is quite outdated, \fmtversion.}
 \typeout{* The WS Book class can only be used with a recent version}
 \typeout{* of LaTeX2e, please upgrade your installation!}
 \typeout{*}
 \expandafter\stop
\else
 \ifnum\expandafter\next\fmtversion\next<199806 \relax
   \typeout{* Warning: }
   \typeout{*}
   \typeout{* Your LaTeX version is outdated, \fmtversion.}
   \typeout{* We believe that it will probably work, but if you encounter}
   \typeout{* problems you will need upgrade your installation.}
   \typeout{*}
   \typein{* Type <return> to continue ...}
   \errortrue
 \else
   \typeout{   ... ok}
 \fi
\fi

\typeout{ }
\typeout{3. Searching for ws-book9x6.cls ... }
\IfFileExists{ws-book9x6.cls}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{* ... ws-book9x6.cls, file not found! }
     \typeout{*}
     \typeout{* Fatal error occurred:}
     \typeout{*}
     \typeout{* The ws-book9x6 class file which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Stopping...}
     \typeout{*}
     \stop
}

\typeout{ }

\typeout{4. Searching for ws-crop9x6.sty ... }
\IfFileExists{ws-crop9x6.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-crop9x6.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-crop9x6 file which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Without this package you will not be able to typeset }
     \typeout{* your book in 9x6 trim size.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{5. Searching for ws-book-har.sty ... }
\IfFileExists{ws-book-har.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-book-har.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-book-har file which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Without this package you will not be able to typeset }
     \typeout{* your references in WS author-date format.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{6. Searching for ws-book-van.sty ... }
\IfFileExists{ws-book-van.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-book-van.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-book-van file which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Without this package you will not be able to typeset }
     \typeout{* your references in WS numbered format.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{7. Searching for ws-book-har.bst ... }
\IfFileExists{ws-book-har.bst}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-book-har.bst, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The BiBTeX style file, ws-book-har.bst which is part of the}
     \typeout{* WS Books distribution must be installed in a directory which}
     \typeout{* is searched by LaTeX.}
     \typeout{*}
     \typeout{* Without this package you will not be able to BiBTeX your references}
     \typeout{* in WS author-date format. If you are not a BiBTeX user you may}
     \typeout{* ignore this warning message.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{8. Searching for ws-book-van.bst ... }
\IfFileExists{ws-book-van.bst}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-book-van.bst, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The BiBTeX style file, ws-book-van.bst which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Without this package you will not be able to BiBTeX your references}
     \typeout{* in WS numbered format. If you are not a BiBTeX user you may}
     \typeout{* ignore this warning message.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }

\typeout{9. Searching for ws-multind.sty ... }
\IfFileExists{ws-multind.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-multind.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-multind package which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the ws-book9x6 class without this package but }
     \typeout{* you can not use multiple indexes.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{10. Searching for ws-book-thm.sty ... }
\IfFileExists{ws-book-thm.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-book-thm.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-book-thm package which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You need this package to typeset your theorems in WS format.}
     \typeout{* Alternate option is `amsmath` package.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }

\typeout{11. Searching for rotating.sty ... }
\IfFileExists{rotating.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... rotating.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The rotating package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to use}
     \typeout{* sidewaysfigure and sidewaystable environments.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "rotating".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{12. Searching for crop.sty ... }
\IfFileExists{crop.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... crop.sty, file not found! }
     \typeout{*}
     \typeout{*}
     \typeout{* The crop package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* This package is required for printing the crop marks.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "crop".}
     \typeout{*}
     \typeout{* Stopping...}
     \typeout{*}
     \stop
}

\typeout{ }
\typeout{13. Searching for hyperref.sty ... }
\IfFileExists{hyperref.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... hyperref.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The hyperref package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to produce a hyper-linked pdf output.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "hyperref".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{14. Searching for boxedminipage.sty ... }
\IfFileExists{boxedminipage.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... boxedminipage.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The boxedminipage package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to use the boxedtxt}
     \typeout{* environment. Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "boxedminipage".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{15. Searching for makeidx.sty ... }
\IfFileExists{makeidx.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... makeidx.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The makeidx package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to generate index.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "makeidx".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }

\typeout{* Finished Testing *}
\typeout{ }
\onerror
\typeout{* Some of the file(s) required by WS was not found.}
\typeout{* Please review the above comments carefully and update your system.}
\typeout{*}
\typeout{* WS files can be downloaded from:}
\typeout{* http://www.worldscientific.com/page/authors/book-stylefiles}
\typeout{*}
\typeout{* Other TeX packages can be downloaded from:}
\typeout{* http://www.ctan.org/search.html}
\typeout{*}
\typeout{* For technical support, please email Rajesh <rajesh@wspc.com.sg>}
\typeout{*}
\typeout{*****************************************************************}
\typein{* Type <return> to continue ...} \else
\typeout{*****************************************************************}
\typeout{*}
\typeout{* All the files and packages required by WS was found,}
\typeout{* you may now proceed LaTeXing your files.}
\typeout{*}
\typeout{* For technical support, please email Rajesh <rajesh@wspc.com.sg>}
\typeout{*}
\typeout{*****************************************************************}
\fi
\stop
\endinput

